AdaTest:Reinforcement Learning and Adaptive Sampling for On-chip Hardware Trojan Detection

This paper proposes AdaTest, a novel adaptive test pattern generation framework for efficient and reliable Hardware Trojan (HT) detection. HT is a backdoor attack that tampers with the design of victim integrated circuits (ICs). AdaTest improves the existing HT detection techniques in terms of scalability and accuracy of detecting smaller Trojans in the presence of noise and variations. To achieve high trigger coverage, AdaTest leverages Reinforcement Learning (RL) to produce a diverse set of test inputs. Particularly, we progressively generate test vectors with high reward values in an iterative manner. In each iteration, the test set is evaluated and adaptively expanded as needed. Furthermore, AdaTest integrates adaptive sampling to prioritize test samples that provide more information for HT detection, thus reducing the number of samples while improving the sample quality for faster exploration. We develop AdaTest with a Software/Hardware co-design principle and provide an optimized on-chip architecture solution. AdaTest's architecture minimizes the hardware overhead in two ways:(i) Deploying circuit emulation on programmable hardware to accelerate reward evaluation of the test input; (ii) Pipelining each computation stage in AdaTest by automatically constructing auxiliary circuit for test input generation, reward evaluation, and adaptive sampling. We evaluate AdaTest's performance on various HT benchmarks and compare it with two prior works that use logic testing for HT detection. Experimental results show that AdaTest engenders up to two orders of test generation speedup and two orders of test set size reduction compared to the prior works while achieving the same level or higher Trojan detection rate.

==> 5_hardware_old.tex <==
\vspace{-0.0em}
\section{\sys{} Hardware Design}  \label{sec:hardware}
\vspace{-0.0em}
Recall that we introduce our innovative RL-based test pattern generation algorithm in Section~\ref{sec:alg}. 
In this section, we demonstrate our hardware design for \sys{} on-chip TPG with optimized hardware cost. 
We discuss the overall architecture of \sys{} hardware and the details of each component in the following of this section. 
% \huc{double check this part with Cheng. }
% \textcolor{red}{At each clock cycle, the TPG produces a test vector that is applied on the PIs of the CUT. }

%% overall hardware design 
\vspace{-0.0em}
\begin{figure*}[ht!]
\centering
 \includegraphics[width=0.9\textwidth]{samples/figs/overall_architecture.png} 
 \vspace{-1.8em}
\caption{\label{fig:arch} Architecture diagram of \sys{} logic testing-based Hardware Trojan Detection. }
\vspace{-0.8em}
\end{figure*}

%%
\noindent {\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{Overall Architecture.}
Figure~\ref{fig:arch} shows our hardware implementation of \sys{} hardware-based Trojan detection. 
Our hardware solution consists of a Test Pattern Generator, the Circuit Under Test, a test controller for the TPG, an input selector for the CUT, and a test output comparator. The functionality of each module is explained below: 
\begin{itemize}
    \item \textit{Circuit Under Test (CUT):} This is the actual circuit that we need to inspect whether a Trojan is inserted.
    \item \textit{Circuit Input Selector (CIS):} This is a multiplexer that selects the input data applied on the CUT. The input data is either the test pattern in the testing stage, or the operation data in the circuit functioning stage.  
    \item \textit{Test Pattern Generator (TPG):} This module generates the sequential test vectors (deterministic in our hardware design) that are searched by \sys{} RL-based adaptive test set generation. Note that \sys{} ensures \textit{high Trojan coverage} while simultaneously \textit{minimizing the number of test patterns}. This indicates that the test generation time on the hardware is also optimized.  
    \item \textit{Test Control Unit (TCU):} It produces control signals for HT detection used by other components: (i) Starting test pattern generation of the TPG; (ii) Selecting the primary inputs of the CUT as the test vectors generated by the TPG; (iii) Activating test response analysis to determine HT existence. 
    \item \textit{Test Response Analyzer (TRA):} This component compares the test responses of the CUT observed from the primary outputs (POs) with the expected ground-truth responses stored in the ROM. A mismatch of test responses reveals the presence of the Hardware Trojan in the CUT.
\end{itemize}


%%
\subsection{\sys{} Test Pattern Generator}
\label{sec:TPG}
Recall that the TPG on the hardware is expected to produce a sequence of deterministic test vectors found by \sys{} adaptive test generation algorithm detailed in Section~\ref{sec:alg}. 
One straightforward implementation is to use a Read-Only Memory (ROM) to store our searched test set. However, the ROM-based solution induces expensive hardware costs. In this paper, we develop an efficient deterministic TPG using a {cyclic Shift Register (SR)}, an {OR-gate network}, a ripple counter, and a multiplexer.

Figure~\ref{fig:cyclic_SR} shows the general overall architecture design of \sys{} framework. 
The cyclic SR has $I$ number of flip flops {where $I$ is the total number of test patterns used in HT detection (i.e., test set size)}.
{The content of the cyclic SR is fed into the OR-gate network to produce the desired sequence of test patterns~\cite{dufaza1993lfsrom}.}
The multiplexer is controlled by the ripple counter whose clock signal is connected to the output of the right-most D flip-flop of the SR. Note that the $\overline{PR}$ and $\overline{CLR}$ signal of the ripple counter are set to $1$.


%% ---- Overall Archic. ----- %%
\vspace{-1.2em}
\begin{figure*}[ht!]
\centering
 \includegraphics[width=0.95\textwidth]{samples/figs/cyclicSR.png} 
 \vspace{-1.3em}
\caption{\label{fig:cyclic_SR} A general architecture of cyclic SR-based TPG for Hardware Trojan detection. }
\vspace{-1.3em}
\end{figure*}


\vspace{0.2em}
{\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{Cyclic Shift Register (SR).} 
A shift register is a cascade of flip-flops (FFs) that share the same clock. The output of each FF is connected to the data input of the next FF in the chain. As such, at each clock cycle, the bit sequence stored in the SR is shifted by one position. This means that the data present at its inputs is shifted in and the last bit in the SR is shifted out.   
A \textit{cyclic SR} is constructed by connecting the last output to the serial input of the SR~\cite{dufaza1993lfsrom}. 
Note that the test vectors generated by conventional LFSRs are randomly ordered. As such, LFSRs are typically used as pseudo-random pattern generators (PRPG)~\cite{wang2002ds}.
Since our RL-based adaptive test set generation (Section~\ref{sec:alg}) produces an ordered sequence of test vectors that are known in the hardware design stage, the cyclic SR-based TPG design is more suitable for our \textit{deterministic} test set generation compared to the LFSR-based solutions.    

% An LFSR is a shift register that consists of memory elements (flip-flops or latches), exclusive OR (XOR) gates, and feedback from different stages.  

{\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{OR-gate Network.} We use an OR-gate network where each output $X_i$ is the logic OR of the content of the connected cyclic SR. 
Figure~\ref{fig:or_net} shows the working mechanism of the OR gate-based network. 
The output $X_i$ can be expressed as follows:
\begin{equation}
    \label{eq:or_net}
    X_i = \sum^I_{j=1} C_{i,j} d_j,
\end{equation}
where the coefficients $C_{i,j}$ indicates the appearance ($C_{i,j}=1$) or non-presence ($C_{i,j}=0$) of a tap from the $j^{th}$ D flip-flop to the $i^{th}$ output. The content of the $j^{th}$ D cell is denoted with $d_j$.   
In general, the $i^{th}$ bit in the test vector $X_i$ is determined by the linear combination of the values in the cyclic SR weighted by the indicator coefficients.    

%% OR gate network %%
\vspace{-1.5em}
\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/or_net.png} 
    \vspace{-1.8em}
    \caption{OR-gate network driven by a four-stage cyclic shift register~\cite{dufaza1993lfsrom}. }
    \label{fig:or_net}
    \vspace{-1em}
\end{figure}


{\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{Map Test Pattern to Connection in OR Gate Network.}
We explain how to generate a test vector of specific content using the cyclic SR and the OR gate network here. 
Let us assume that the cyclic SR is initialized such that only the leftmost D flip-flop is filled with one and all the other elements are filled with zeros. 
In this case, the element with a value of one is shifted right by one position after each clock cycle. 
Note that this value of one returns to its original location (i.e., the leftmost position) after $I$ clock cycles due to the circular property of the cyclic SR ($I$ is the number of D flip-flops in the SR). As such, the cyclic SR can take in total $I$ states with this initialization~\cite{dufaza1993lfsrom}.
Let us assume that the $k^{th}$ D cell of the SR has the element of one, then Equation~(\ref{eq:or_net}) can be simplified as follows: 
\vspace{-0.5em}
\begin{equation}
    \label{eq:Xi}
    X_i = C_{i,k},
    \vspace{-0.5em}
\end{equation}
because we have $d_k=1$ and $d_j =0$ for any $j \neq k$. 
This means that the $i^{th}$ bit of the output of the OR-gate network is determined by the coefficients $C_{i,j}$ (indicator of the tap existence). Therefore, we can conclude that there is a \textit{deterministic mapping} between the sequence generated by the OR-gate network and the network connection. 
For the OR-gate network shown in Figure~\ref{fig:or_net} with an initialization of $\left\{d_1, d_2, d_3, d_4\right\} = \left\{0, 0, 1, 0\right\}$, the following sequence of test vectors will be generated: $\left\{1,1,0\right\}$, $\left\{0,1,0\right\}$, $\left\{0,1,1\right\}$, $\left\{1,0,1\right\}$. 

Our architecture design leverages this observation to build on-chip TPG for \sys{}.
Particularly, we first perform adaptive test pattern exploration for the given CUT using Algorithm~\ref{alg:adaptive_rl}. 
The obtained test set is then generated by our hardware TPG (Figure~\ref{fig:cyclic_SR}) by configuring the tap existence of the cyclic SR based on the desired sequential test vectors. 

%% 
\vspace{0.3em}
{\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{Scaling to Test Large Circuits.}
Our architecture design of the TPG (Figure~\ref{fig:cyclic_SR}) is highly \textit{modular}, thus is \textit{scalable} to complex circuits that require a large number of test patterns (meaning that the size of the cyclic SR $I$ needs to be large). 
Mathematically, the test pattern set of the CUT is a 2D matrix of dimension $I \times \#PIs$ where $I$ is the total number of test vectors and $\#PIs$ is the number of primary inputs (PIs) of the CUT. 
These two dimensions allow us to partition the test set in two ways. 
The first modularization approach is to \textit{partition} the desired long test set into multiple smaller test set for the CUT (i.e., dividing along the first dimension of the test set matrix: $I=\sum_i I_i$). In this case, a smaller cyclic SR with $I_i$ D cells can be used to drive the OR-gate network and generate a subset of the test patterns for the CUT.  
% the desired long sequence into multiple \textit{sub-sequences} of equal length and building an OR gate sub-network for each sub-sequence (i.e., divide along the first dimension of the test set matrix $I=\sum I_i$). 
% Note that each OR gate sub-network is connected with its corresponding cyclic SR (length shorter than \sys{}'s test set size). 
% An additional multiplexer is used to select the sub-sequence for current processing. 
An additional multiplexer is used to select the subset of test patterns for current processing. 
The ripple counter detects that the unique 1 of the SR finishes one full cycle (from the leftmost to the rightmost D cell) and requests the next sub-sequence. 
It is worth noting that the size of each cyclic SR $I_i$ (i.e., the number of D flip-flops) is a \textit{tunable design parameter} that affects the hardware cost. This is due to the fact that a smaller number of D cells for each test subset generation requires a larger multiplexer to coordinate the generation of the full test set for the CUT.
As such, we can find the \textit{optimal} number of D cells of a cyclic SR by modeling the hardware cost with respect to the number of D flip-flops inside each cyclic SR. 
% number of three key components: SR, OR gate, and MUX. 


% An alternative solution to detect potential HTs on large-scale SoCs 
An alternative test set partitioning method is to divide the CUT into multiple regions by exploring the \textit{independence} between signal clusters~\cite{chen2020flowtrojan} (i.e., dividing along the second dimension of the test set matrix: $\#PIs=\# \bigcup_j PIs_j$).
After \textit{circuit partitioning}, \sys{} can generate the test set based on Section~\ref{sec:alg} for each sub-netlist of the CUT individually. The corresponding hardware design for HT detection of each sub-circuit can be derived from the general architecture in Figure~\ref{fig:arch}. 
Note that for a given CUT, the number of independent signal clusters is a \textit{deterministic} value instead of a tunable parameter in the first solution discussed above (i.e., chunking the test set). 
The \textit{modular design} principle of \sys{} reduces the HT {detection time} since each sub-circuit can be tested in \textit{parallel}.
% and the \textit{hardware cost} simultaneously.  


%%
\subsection{\sys{} Controller Unit}  \label{sec:control_unit}
There are two modes for a CUT equipped with \sys{} design: \textit{test mode} and \textit{operational mode}.  
When the test mode is enabled by the \textit{`Test Control Unit'} shown in Figure~\ref{fig:arch}, the CUT undergoes our logic testing-based HT detection.   
In this mode, the Circuit Input Selector in Figure~\ref{fig:arch} is configured to choose the test patterns from the TPG and apply them on the CUT. 
In the meantime, the Test Response Analyzer is activated to collect the test outputs of the CUT and compare them with the expected values for HT detection. 
{Note that test generation and test response analysis can be performed \textit{concurrently} in the test mode.}
% \huc{Need to revise and check correctness?}


For large-scale circuits, \sys{} logic testing-based HT detection can be performed on the \textit{partitioned netlist} using our modular design principle. 
Recall that we suggest two methods to partition test patterns in Section~\ref{sec:TPG}: each cyclic SR-driven OR-gate network generates a smaller number of test vectors for the complete CUT, or generate the desired number of test vectors for a region of the CUT.
% dividing the test set along the dimension of the tuning the number of D flip-flops leverage circuit signal independence. 
% In this scenario, multiple cyclic SR-driven OR-gate networks will generate test patterns for each sub-circuit independently. 
% Let us assume we use the second circuit partitioning approach. 
{There are two options to detect whether a HT in inserted in the original CUT: \textit{(i) Distributed testing.} In this setting, multiple circuit input selectors and test responses analyzers are devised for each sub-netlist with the corresponding test control unit in control. 
\textit{(ii) Centralized testing.} The circuit input selector is shared among all TPG modules with a single control line. A central test control unit coordinates all the TPG modules as well as the aggregation of their outputs at the circuit input selector. 
After applying the test patterns on the CUT, the test responses from each CUT sub-netlist are collected and compared with the ground-truth values stored in the ROM. In this case, only a single test response analyzer is used to perform HT detection.}


It is straightforward to see that the \textit{distributed testing} approach features computation \textit{parallelism}, thus requires shorter detection time at the cost of higher hardware resource consumption. 
The \textit{centralized testing} method has smaller hardware complexity while it works in a \textit{sequential} manner, suggesting a longer detection time. 
This \textit{trade-off} between HT detection {latency} and {hardware cost} can be explored by the circuit tester based on his desired detection speed and hardware resource budget.  
% Note that the \textit{HT detection} process is typically considered as an \textit{offline} procedure performed before the CUT enters the normal operational mode. 
% \huc{control signals generated by FSM?? different states and corresponding control table for the  TPG, CIS, and TRA}


\subsection{\sys{} Test Response Analyzer}
There are two inputs to the test response analyzer (TRA): the actual test responses of the CUT, and the ground-truth test outputs from the ROM. 
When the TRA is enabled by the test control unit, a \textit{comparator} is used to check if the test output is equal to the expected value in the ROM.
% \textcolor{red}{The test response signals of the CUT are originally in the parallel form. The response data is first cached and converted to the serial format before they enter the test response analyzer. }
A complex circuit can have a large number of primary outputs, meaning that the test output might be longer than the expected values read from the ROM in one clock cycle. 
In this case, multiple rows of the ROW are accessed in order and compared with the corresponding segment of the long test response sequence. 
To provide the testing capability for large circuits, our design of the TRA integrates a \textit{buffer} that can store the test response of the CUT for a sufficient number of clock cycles such that the bit-wise comparison with the ROM read can be completed. 
The buffer can be implemented with the right shift register. % without pipelining 
If the test response is shorter than the data size that can be read from the ROM in a single cycle, then no buffer is needed. 


Let us take the $des$ benchmark of ISCAS'85 with $\#POs=245$ as an example and assume that the ROM can output a 32-bit data in one cycle given its address.
In this case, the buffer for the test response needs to hold data for $[245/32]=8$ cycles for each comparison. 
The TPG in Figure~\ref{fig:arch} needs to satisfy the \textit{timing constraint} that the interval between the arrival of each consecutive test response at the TRA is larger than the comparison time of one full test output with the expected values. 
Note that the arrival interval of test outputs is the runtime of two main steps: test input generation by the cyclic SR-driven OR-gate network, and CUT execution with the test vector applied at its PIs.
% The TPG generates a new test vector for the CUT and apply it after the completion of one comparison. 


The collected test responses might be too large to be analyzed on-chip for complex circuits. In this case, the test outputs can be {compressed} as a \textit{signature}. 
With response compaction, the signature extracted from the CUT and the one from the Trojan-free circuit reveals the presence of a HT. 

% \subsection{Case Study: HT Detection of UART}
% {\tikz\draw[black,fill=black] (-0.5em,-0.5em) rectangle (-0.2em,-0.2em);} \textbf{Case Study: HT Detection of UART.}
% In this section, we demonstrate a case hardware design of \sys{} for HT detection of an 8-bit universal asynchronous receiver transmitter (UART). 
% A UART is a device for asynchronous serial communication with configurable data formats and transmission speeds. 
% As an example of CUTs, the UART monitors the correctness of all the received data bytes. 
% We use a UART with the following components: status register, transmitter, receiver, and baud rate generator as in~\cite{manjesh2014fpga}. 
%% transmitter 
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.75\textwidth]{samples/figs/transmitter.png} 
%     \vspace{-1.3em}
%     \caption{Example design of a UART transmitter.}
%     \label{fig:transmitter}
% \end{figure}


%% receiver 
% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.85\textwidth]{samples/figs/receiver.png} 
%     \vspace{-1.3em}
%     \caption{Example design of a UART receiver.}
%     \label{fig:receiver}
% \end{figure}



